DeepVulSeeker: A Novel Vulnerability Identification Framework via Code Graph Structure and Pre-training Mechanism

Software vulnerabilities can pose severe harms to a computing system. They can lead to system crash, privacy leakage, or even physical damage. Correctly identifying vulnerabilities among enormous software codes in a timely manner is so far the essential prerequisite to patch them. Unfortantely, the current vulnerability identification methods, either the classic ones or the deep-learning-based ones, have several critical drawbacks, making them unable to meet the present-day demands put forward by the software industry. To overcome the drawbacks, in this paper, we propose DeepVulSeeker, a novel fully automated vulnerability identification framework, which leverages both code graph structures and the semantic features with the help of the recently advanced Graph Representation Self-Attention and pre-training mechanisms. Our experiments show that DeepVulSeeker not only reaches an accuracy as high as 0.99 on traditional CWE datasets, but also outperforms all other exisiting methods on two highly-complicated datasets. We also testified DeepVulSeeker based on three case studies, and found that DeepVulSeeker is able to understand the implications of the vulnerbilities. We have fully implemented DeepVulSeeker and open-sourced it for future follow-up research.

==> discuss.tex <==
%Although it is shown in the evaluation part that our proposed approach and implementation can have a sound effect against dangerous smart home apps, however, as aforementioned, our approach cannot defend against open-port based attacks due to the reasons illustrated in Section~\ref{sec:background}. Fortunately, there are multiple alternatives that may have the potential to mitigate these attacks. 
%\begin{itemize}
%\item \textbf{Inhibiting Dictionary Attacks.} Dictionary attacks is the first step that Mirai took to compromise IoT devices~\cite{mirai}. Therefore, inhibiting dictionary attacks may effectively hinder Mirai and similar botnets exploiting weak credentials. Currently, multiple solutions have been proposed to inhibit the dictionary attacks from different aspects~\cite{bontrager2018}\cite{2016wuhiera}. Yet, these solutions are mainly designed for general-purpose computing systems. Whether or not they can be migrated to the embedded systems needs to be further scrutinized.
%
%\item \textbf{Code-Level Vulnerability Discovery.} Sophisticated botnets (e.g., IoTReaper) exploits a number of zero-day vulnerabilities to compromise IoT devices~\cite{greenberg2017reaper}. Therefore, code-level bug searching techniques may serve as ideal solutions to mitigate the zero-day based open-port attacks~\cite{shoshitaishvili2015firmalice}\cite{muench2018you}\cite{Zheng2017usenix}.
%
%\item \textbf{Hardware-Assisted Approaches.} Some zero-day vulnerabilities may be too complicated to be uncovered using merely the static code-level analysis. In this case, leveraging hardware as an assistant to isolate sensitive information/codes from the insensitive ones can constrain the damages brought by the zero-day vulnerabilities~\cite{Frassetto2018imix}\cite{weiser2019timber}. 
%\end{itemize}
